Multi-Source Domain Adaptation with Mixture of Experts

We propose a mixture-of-experts approach for unsupervised domain adaptation from multiple sources. The key idea is to explicitly capture the relationship between a target example and different source domains. This relationship, expressed by a point-to-set metric, determines how to combine predictors trained on various domains. The metric is learned in an unsupervised fashion using meta-training. Experimental results on sentiment analysis and part-of-speech tagging demonstrate that our approach consistently outperforms multiple baselines and can robustly handle negative transfer.

==> tables/amazon-entropy-ablation.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|cc|cc}
%     \hline
%     & \multicolumn{2}{c}{MOE} & \multicolumn{2}{c}{MOE-A} \\
%     Setting & w/o $\mathcal{R}_h$ & w/ $\mathcal{R}_h$ & w/o $\mathcal{R}_h$ & w/ $\mathcal{R}_h$ \\
%     \hline
%     D,E,K-B & 78.72 & 79.42 & 80.36 & 80.87 \\
%     B,E,K-D & 82.68 & 83.35 & 83.58 & 83.99 \\
%     B,D,K-E & 84.69 & 86.62 & 85.94 & 86.38 \\
%     B,D,E-K & 87.47 & 87.96 & 87.97 & 88.06 \\
%     \hline
%     D,E,K-B & 86.80 & 87.55 & 87.25 & 87.85 \\
%     B,E,K-D & 87.80 & 87.85 & 86.45 & 87.65 \\
%     B,D,K-E & 88.50 & 89.20 & 88.90 & 89.50 \\
%     B,D,E-K & 89.95 & 90.45 & 90.75 & 90.45 \\
%     \hline
%     \end{tabular}
%     \caption{Ablation test of entropy regularizer on \textsc{Chen12}.}
%     \label{tab:analysis-entropy}
% \end{table}
